Cache-Oblivious Parallel Convex Hull in the Binary Forking Model

We present two cache-oblivious sorting-based convex hull algorithms in the Binary Forking Model. The first is an algorithm for a presorted set of points which achieves $O(n)$ work, $O(\log n)$ span, and $O(n/B)$ serial cache complexity, where $B$ is the cache line size. These are all optimal worst-case bounds for cache-oblivious algorithms in the Binary Forking Model. The second adapts Cole and Ramachandran's cache-oblivious sorting algorithm, matching its properties including achieving $O(n \log n)$ work, $O(\log n \log \log n)$ span, and $O(n/B \log_M n)$ serial cache complexity. Here $M$ is the size of the private cache.

==> algorithm_docs/angularElimination.tex <==
\section{A Paramaterized Work-Span Tradeoff Algorithm}\label{sec:angular}

%To overcome the limitations of our previous algorithms spans, 
In this section we present a recursive tradeoff algorithm for finding 2D convex hulls which achieves $O(k \log n)$ span with $O(n ^{1+\frac{1}{k}} \log n)$ work, where $k$ is a positive integer. This allows us to achieve $O(\log n)$ span for any constant value of $k$, so a small work increase is incurred as a result. In addition to the primitives we have described, the algorithm makes use of two subroutines. The first, which we call \textit{DominatingRange} determines for a given wave and a set of other waves the range for which the given wave dominates the others. The second, which we refer to as just \textit{BaseCase}, uses that subroutine to determine the active ranges of each wave in the upper envelope. We finally bring them all together to create a recursive algorithm that goes a parameterized depth before calling the Base Case and then using the subproblem solutions to decrease the number of waves individual wave needs to be compared against. 

\subsection{Determining the dominating range}
\textit{DominatingRange} (Algorithm \ref{alg:DominatingRange} in Appendix \ref{sec:pseudocodes}) takes a particular wave, $wave$, and a set of waves, $W$ and determines over what range $[0,2\pi ]$ $wave$ has a $R$ value that is greater than all those of $W$. It also determines which wave overtakes it at the end of the range, specifically the wave which intersects it at an endpoint of its range and has a greater slope at that intersection. This will be useful for determining neighbors of waves that are in the upper envelope.

We find this recursively. At the base case, $|W| = 1$ so we compare $wave$ to one other wave in W. This can be done in constant time by finding the intersection points and determining which side of the split $wave$ is above the other. Above this level, we find the intersection of the two ranges given by the recursive calls using the \textit{CommonRange} primitive.

\begin{theorem}
For $n$ sine waves of the form $x \cos \theta + y \sin \theta$, Algorithm 4 (Dominating Range) finds the range over which one dominates all the others in $\Theta(\log n)$ span and $\Theta(n)$ work.
\end{theorem}
\begin{proof}


\begin{equation*}
  \textrm{Work,~} W(n)=\begin{cases}
    \Theta(1), & \text{if $n$ is 1}.\\
    2W(\frac{n}{2})+\Theta(1), & \text{otherwise}.
  \end{cases}
\end{equation*}

\begin{equation*}
 \textrm{Span,~} S(n)=\begin{cases}
    \Theta(1), & \text{if $n$ is 1}.\\
    S(\frac{n}{2})+\Theta(1), & \text{otherwise}.
  \end{cases}
\end{equation*}
This follows from the fact that each primitive function performs $O(1)$ work.
Using Master's theorem, we get $\Theta(n)$ work and $\Theta(\log n)$ span.


\end{proof}


\subsection{Base case of the algorithm}
Our base case algorithm essentially applies \textit{DominatingRange} to each individual wave for the entire set of waves. It does this in parallel for all waves in $W$, which amounts to $n$ calls of \textit{DominatingRange} running alongside each other. At this point, we have a linked list representation of the upper envelope. We can transfer these elements in parallel to an array by determining their order and then placing them into the array in parallel. We determine the rank using a list ranking algorithm, with the one modification being that the ranks of waves with empty ranges are set to $n$ to start to avoid any possibility of accidentally being added into the array.

For both the base case algorithm and the main algorithm, we use Blelloch et al.'s \cite{BlellochFiGuSu2019} adaptation of Wyllie's list ranking algorithm, which performs $O (n \log n)$ work in $O(\log n)$ span. Since this subroutine uses Test-and-Set (TS), this algorithm as a whole does not apply to the binary-fork join model.
%, but if a linked-list representation is allowed then the base case algorithm itself has the same bounds in the binary-fork join model.

\begin{theorem}
For $n$ sine waves of the form $x \cos \theta + y \sin \theta$, Algorithm 5 (the Base Case of Angular Elimination) finds the upper envelope in $\Theta(\log n)$ span and $\Theta(n^2)$ work.
\end{theorem}
\begin{proof}
Since \textit{DominatingRange} performs $\Theta(n)$ work and this is performed once for every wave in $W$, the total work must be $\Theta(n^2)$, which dominates the $O(n \log n)$ list ranking and $O(n)$ array assignments.

Since \textit{DominatingRange}, list ranking, and spawning in threads all have $\Theta(\log n)$ span, it follows that the entire algorithm must have $\Theta(\log n)$ span in total.
\end{proof}


\subsection{Recursive structure}
The final algorithm combines \textit{DominatingRange} and the base case to form a parameterized recursive algorithm which allows a trade-off between optimal span for $k = O(1)$ and optimal work for $k=\log n$.

The structure of its recursion is very similar to Goodrich and Ghouse's \cite{Ghouse91fastrandomized} "inductive" convex hull algorithm which performs $O(k)$ span using $n^{1+\frac{2}{k}}$ processors in CRCW PRAM model. We split the waves into groups of size $O(n^{\frac{1}{k}}$, apply our algorithm on these subgroups, and decrease the $k$ value by 1 for these calls. If $k$ is 1 or less, then we use the base case algorithm.

After finding the envelopes of the subproblems, we apply \textit{DominatingRange} to determine the range for which each wave is part of the upper envelope. From the subproblem solutions, each wave now has some active range or has already been eliminated. For each subproblem envelope, the wave has some subsection that it may overlap with. We find this subsection with binary search and then apply \textit{DominatingRange} to only the set of waves in that subsection. We do this from every wave to every subproblem envelope and collect the resulting ranges from each of these in an array. We then find the intersections of all these ranges to get the final range for which each wave is dominant. Just as with the base case, we apply list ranking to return the upper envelope in array form.

\begin{theorem}
For $n$ sine waves of the form $x \cos \theta + y \sin \theta$, Algorithm 6 (Angular Elimination) finds the upper envelope in $\Theta(k \log n)$ span and $O(n^{1+\frac{1}{k}} \log n)$ work, where $k \in [1, \log{n}]$ is an integer.
\end{theorem}

\begin{proof}
Let $W(n, k)$ be the work and $S(n, k)$ be the span of the algorithm for an input size $n$ and parameter value $k$. Then

\begin{equation*}
  W(n,k)=\begin{cases}
    \Theta(n^2), & \text{if $k \leq 1$}.\\
    n^{\frac{1}{k}}W(n^{\frac{k-1}{k}},k-1)+\Theta(n^{1 + \frac{1}{k}} \log n), & \text{otherwise}.
  \end{cases}
\end{equation*}

\begin{equation*}
 S(n,k)=\begin{cases}
    \Theta(\log n), & \text{if $k \leq 1$}.\\
    S(n^{\frac{k-1}{k}},k-1)+\Theta(\log n), & \text{otherwise}.
  \end{cases}
\end{equation*}
The recurrences follow since for $k>1$, the work and span are equal to that of the division into subproblems plus the merging of those subproblems. The subproblem work and span comes from there being $n^{\frac{1}{k}}$ subproblems of size $n^{\frac{k-1}{k}}$.

For the merging, first, we consider the work. We iterate over the set of all waves. Each of these then compares themself against $n^{1/k}$ subproblem solutions. Finding the leftmost and rightmost curves with the overlapping range can be done in $\Theta(\log n)$ time using binary search. This part takes $\Theta(n^{1 + \frac{1}{k}} \log n)$ work.

Applying \textit{DominatingRange} to the range between can have worst-case $O(n^{k-1}{k})$ work, but this would require that there are $O(n^{k-1}{k})$ curves that overlap with the wave we are analyzing. If that is the case, then only 2 of those curves can overlap with the ranges of the other waves in the same subproblem as the wave we are analyzing. which means we can amortize this work. For the $n^{1/k}$ subproblem solutions, we perform $(n^{1/k}-1) \cdot \Theta (n^{\frac{k-1}{k}})$ work, which multiplies out to be $\Theta(n^{1 + \frac{1}{k}})$ work, which is dominated by the previous work.

For span, all operations take $\Theta (\log n)$ time including spawning threads, so the contribution of the merge is $\Theta (\log n)$.

The recurrences can be shown to be $S(n,k) = O(k \log n)$, 
and $W(n,k) = O(n^{1+\frac{1}{k}} \log n)$ through induction on $k$. Evaluating at $k = 1$, we have $S(n,1) = \Theta(\log n) = \Theta (1 \cdot \log n)$ and $W(n,1) = O(n^2) \in O(n^{1+1/1} \log n)$. Assuming that for some $k_0 \geq 1$ the bounds hold, we can show that the bounds hold for $k_0 +1$. 

\begin{align*}
S(n,k_0 +1) &= S(n^{\frac{k_0-1}{k}},k_0) + \Theta (\log n)\\
 & = \Theta (k_0 \log (n^{\frac{k_0-1}{k_0}}) + \Theta (\log n)\\
 &\leq c_1 (k_0-1) (\log (n)) + c_2 \log(n)\\
 &\leq (k_0+1)\log n, \text{ for } c_1=1,c_2=2
\end{align*}
And the same applies for work:
\begin{align*}
    W(n,k_0 +1) &=  n^{\frac{1}{k_0 +1}} W(n^{\frac{k_0}{k_0 +1}},k_0)+ \Theta(n^{1+\frac{1}{k_0 +1}} \log n ) \\
    & = O \left( n^{\frac{1}{k_0+1}} \cdot  n^{\left(\frac{k_0+1}{k_0} \right) \left(\frac{k_0}{k_0+1} \right)} \log \left( n ^ \frac{k_0}{k_0+1}\right)\right)\\
     & + \Theta(n^{1+\frac{1}{k_0+1}} \log n)\\
     &\leq c_1 \frac{k_0}{k_0+1} n^{1+\frac{1}{k_0+1}} \log n + c_2 n^{1+\frac{1}{k_0+1}} \log n \\
     &\leq n^{1+\frac{1}{k_0+1}} \log n, \text{ for } c_1=0.5,c_2=0.5
\end{align*}
Therefore, Angular Elimination performs $O\left(n^{1+\frac{1}{k}} \log n \right)$ work with $O(k \log n)$ span.
\end{proof}

Since we used induction on $k$ starting with 1 as our base case, $k$ is restricted to positive integers. Additionally, for any $k> \log n$, we incur more span with no improvements in work, which at $k = \log n$ becomes $O(n \log n)$. Thus we define the parameter $k$ to be a positive integer in the range $[1,\log n]$.



==> algorithm_docs/divide-and-conquer.tex <==
\section{Divide and conquer with parallel merge}\label{sec:divide-and-conquer}
%main description shows the result
We propose a straightforward divide-and-conquer approach which has $O(n\log n)$ work and $O(\log^2 n)$ span, using the Positive Curve Form representation.
%high level idea of the algorithm
In this divide-and-conquer algorithm, we partition the collection of the $n$ sinusoidal waves into two subsets of roughly equal size. We recursively compute the upper envelopes of these two subsets. After getting these two upper envelopes, we parallel merge them into an upper envelope for these $n$ waves. (If needed, please see~\cite{fogel2012cgal} for the detailed implementation of the serial version of this algorithm.)

%describe the details of the algorithm z

In the merge routine, we start by identifying dividing waves for both sets, $A$ and $B$, that would split each of them into subsets of size $\log n$. We then find the rank of these splitting points (i.e., ranks of $A$'s splitting points in $B$ and $B$'s splitting points in $A$) in parallel using binary search. Now we examine each subset of A partitioned by the dividing points for A and its counterpart in B in parallel. If the corresponding subset in B is at most size $\log n$, then run the serial algorithm on the pair. Elsewise, we split the B subset using whichever splitting points from before are in its range and do a serial merge with their counterparts in A. Afterwards, we just need to check at the pivot points to determine the points of intersection for the waves at the boundaries of the subsets. We go into further detail about the necessity of this step as it pertains to the Multiway Merge algorithm \ref{sec:multiway}.
%----------------------------------------------------------------
%pseudocode


\begin{algorithm}
\small
\caption{Divide-and-Conquer with Parallel Merge}\label{alg:divide-and-conquer2}
\KwData{$W$, a set of $n$ sine waves of $x \cos \theta + y \sin \theta$}
\KwResult{The convex hull, in a circular doubly linked list}

\SetKwFunction{DivideAndConquer}{Divide-And-Conquer}
\SetKwProg{Fn}{function}{:}{}

\Fn{\DivideAndConquer(W)}{
$A \gets W[0], W[1], ... W[n/2-1]$\;
$B \gets W[n/2], W[n/2+1], ... W[n-1] $ \;
Merge(DivideAndConquer(A), DivideAndConquer(B),n/2)\;
}
\Fn{Merge(A,B,n)} {
    $A_S \gets$ every $\log n$th wave in A\;
    $B_S \gets$ every $\log n$th wave in B\;
    \textbf{parallel for each} $a_i \in A_S$ determine its rank in B\; 
    \textbf{parallel for each} $b_i \in B_S$ determine its rank in A\; 
    \textbf{parallel} \ForEach {$i = 0, i < n/\log n$}{
    \textbf{if} $a_{i+1}.rank - a_i.rank \leq \log n$ \textbf{then} apply serial merge\;
    \Else {
        Identify the smallest $b_j$ larger than $a_i.rank$\;
        Identify the largest $b_k$ smaller than $a_{i+1}.rank$\;
        \textbf{parallel for each } subset partitioned by $b_j \leq b_p \leq b_k$, \textbf{do} apply serial merge with its counterpart in A\;
        Determine the intersections between the waves on either side of each $b_p$ and adjust the start angles accordingly.\;
    }
    }
    Determine the intersections between the waves on either side of each $a_i$ divider and adjust the start angles accordingly.\;
    
}
\end{algorithm}

\begin{theorem}
Given $n$ sine waves of the form $x \cos \theta + y \sin \theta$, Algorithm~\ref{alg:divide-and-conquer2} outputs the upper envelope in  $O(n\log n)$ work and $O(\log^2 n)$ span.
\end{theorem}
\begin{proof}
We know the parallel merge must have $\Theta(n)$ work. This is because we do $2n/\log n$ binary searches and then apply the serial merge algorithm, which has $O(n)$ work on all the points at some point along the hull. We also know that the merge has $\Theta(\log n)$ span because running the serial algorithm on sets of size at most $2 \log n$, the binary searches and spawning the threads costs $\Theta (\log n)$ span. Based on the recursive design, our algorithm has the following two recurrence equations for work and span.
\begin{equation*}
  \textrm{Work,~} W(n)=\begin{cases}
    \Theta(1), & \text{if $n$ is 1}.\\
    2W(\frac{n}{2})+\Theta(n), & \text{otherwise}.
  \end{cases}
\end{equation*}

\begin{equation*}
\textrm{Span,~} S(n)=\begin{cases}
    \Theta(1), & \text{if $n$ is 1}.\\
    S(\frac{n}{2})+\Theta(\log n), & \text{otherwise}.
  \end{cases}
\end{equation*}

Solving, $W(n) = \Theta(n\log{n})$ and $S(n) = \Theta(\log^2{n})$

\end{proof}



%TODO: analysis check correctness first 


%reference
\iffalse
detailed implementation~\cite{fogel2012cgal}
the book~\cite{sharir1995davenport}

standard~\cite{mikhail1985some,hart1986nonlinearity}

Hershberger
~\cite{hershberger1989finding}
A straightforward divide-and-conquer approach, as described in Section 10.1, yields an algorithm
for constructing the envelope of curves in the plane with running time that has a multiplicative
log factor over the worst-case complexity of the envelope. Hershberger~\cite{hershberger1989finding} improved
this algorithm slightly, such that for segments, for example, it runs in worst-case optimal time
O(n log n). (Without Hershberger’s improvement, the standard divide-and-conquer algorithm runs
in time$O(n\alpha(n) \log n)$.~\cite{mikhail1985some,hart1986nonlinearity})


\begin{algorithm}
\caption{Divide-and-Conquer}\label{alg:divide-and-conquer}
\KwData{$S$, a set of $n$ points in the 2D plane, stored in an array}
\KwResult{The convex hull, in a circular doubly linked list}

\SetKwFunction{DivideAndConquer}{Divide-And-Conquer}
\SetKwProg{Fn}{function}{:}{}
\Fn{\DivideAndConquer{:}}{
    \textbf{if}{ n = 1} \textbf{then}
    {
        \Return S\;
    }
    $S_1 \gets $ elements $0, ... \lfloor n/2-1 \rfloor$ of S\;
    $S_2 \gets $ elements $\lfloor n/2 \rfloor, ... n-1$ of S\;
    $A \gets$ Divide-and-Conquer($S_1,\lfloor n/2 \rfloor$)\;
    $B \gets$ Divide-and-Conquer($S_2,\lceil n/2 \rceil $)\;
    \Return Merge(A,B)\;
}

\SetKwFunction{Merge}{Merge}
    \Fn{\Merge{$A,B$}}{
    \textbf{if} {$A.size \le B.size$ } \textbf{then} \Return Merge(B,A)\;
    \textbf{if} {$B.size = 0$} \textbf{then} {\Return A\;}
    $pivotCurve \gets A[\lfloor A.size/2 \rfloor]$\;
    $pivot \gets$ middle $\theta$ value of $pivotCurve$\;
    $pivotOpposite \gets$ curve in $B$ for $\theta = pivot$\;
    $H \gets \{ \}$\;
    $I \gets$ Intersections($pivotCurve$,$pivotOpposite$)\;
    \If {I[0] \text{in range of both}}
    {
        $H$.add(MaxSlope($pivotCurve$,$pivotOpposite$,I[0]))\; 
        $H$.add(MinSlope($pivotCurve$,$pivotOpposite$,I[0]))\;
    }
    \If {I[1] \text{in range of both}}
    {
        $H$.add(MaxSlope($pivotCurve$,$pivotOpposite$,I[1]))\;
        $H$.add(MinSlope($pivotCurve$,$pivotOpposite$,I[1]))\;
    }
    \If{H is empty}{
        $H$.add(MaxVal($pivotCurve,pivotOpposite, pivot$)
    }
    \Return Merge($A_1,B_1$), H, Merge($A_2,B_2$)\;
    
}
\end{algorithm}


%----------------------------------------------------------------
% show the work and span
\begin{theorem}
Given $n$ points in a plane, Algorithm~\ref{alg:divide-and-conquer} outputs its Convex Hull in  $O(n\log n)$ work and $O(\log^3 n)$ span. To be specific, it outputs these extreme points of the convex hull.
\end{theorem}
\begin{proof}
We know that parallel merge has $\Theta(n)$ work and $\Theta(\log^2 n)$ span. Based on the recursion design, our algorithm has the following two recursion equations for work and span.
\begin{equation*}
  W(n)=\begin{cases}
    \Theta(1), & \text{if $n$ is 1}.\\
    2W(\frac{n}{2})+\Theta(n), & \text{otherwise}.
  \end{cases}
\end{equation*}

\begin{equation*}
 S(n)=\begin{cases}
    \Theta(1), & \text{if $n$ is 1}.\\
    S(\frac{n}{2})+\Theta(\log^2 n), & \text{otherwise}.
  \end{cases}
\end{equation*}
Using Master theorem, we get $\Theta(n)$ work and $\Theta(\log^2 n)$ span.

\end{proof}





\fi



==> algorithm_docs/presorted.tex <==


\section{A Cache-Optimal \texorpdfstring{$O(\log n)$}{O(log n)} Span Algorithm for Presorted Points}

We propose a cache-oblivious divide-and-conquer algorithm for finding the upper convex hull of an array of presorted points. The algorithm achieves $O(\log n)$ span with $O(n)$ work and $O(n/B)$ cache misses, which is optimal in all respects for the binary-forking model. It uses an approach similar to that used by Attallah and Goodrich's \cite{ATALLAH1986} $O(n \log n)$ work algorithm but splits the input into fewer subproblems ($n^{1/5}$ as opposed to $n^{1/2}$) and delays the removal of points that have been found to be strictly inside the hull until all subproblems have been solved.
The pseudocode is given in Algorithm \ref{alg:presorted}. We will start by giving a very general overview and then describing the data formatting we use to make this work.

\subsection{Overview}
Our algorithm is similar to Atallah and Goodrich \cite{ATALLAH1986}'s $O(n \log n)$ work algorithm, but we manage to reduce work and cache misses by decreasing the number of subproblems at each recursion layer and by using an external data structure which we refer to as a "divider array" to allow us to amortize the work required to eliminate points from the hull. We use an $n^{1/5}$-way divide and conquer scheme, splitting the input into subproblems of size about $n^{4/5}$ until we reach a size of $\log n$. At size $\log n$, we simply use a serial algorithm such as Andrew's \cite{ANDREW1979216} variant of the Graham Scan for x-sorted points. In addition to a size $n$ array $A$ for the input points, we use a size $\frac{4n}{\log n}$ array $D$ to maintain what we call "dividers". "Dividers" are a representation for marking alternate regions of points which cannot be on the convex hull and those which are still being considered. So the points which are between a "left" and a "right" divider are considered by the algorithm to be deleted without needing to use $O(n)$ work to explicitly rearrange the array. At each recursion level, we compare the $n^{1/5}$ subproblems as in Atallah and Goodrich \cite{ATALLAH1986}: storing all pairwise common tangents in a tangent array $T$ and compare their slopes. After comparing the slopes, we determine the points that will remain from a particular subproblem and add dividers to the divider array to indicate which points must be deleted. Using the dividers, we mark the points that have to be deleted and continue up to the next recursion layer. Once all points that must be deleted are marked, we delete them all at the end and return the final array of extreme points in sorted order.


\subsection{Data Structure}

All of our data is stored in 3 different types of arrays: \textbf{points}, \textbf{dividers}, and \textbf{tangents}. All three element types are of constant size, so each array has size linear in the number of elements.

\textbf{Points} are based on the input, with some extra attributes assigned to each point so that the algorithm can keep the point in its position after being marked for deletion without impeding the ability to merge the upper hulls of subsections that it is a member of. In addition to $x$- and $y$-coordinates, the point contains a RANK integer flag which is initialized to 1 and two pointers to dividers called LEFTPAR and RIGHTPAR, intuitively the two dividers which marked it for deletion, one to its left and one to its right. LEFTPAR and RIGHTPAR are initialized to NULL.

\textbf{Dividers} indicate which points need to be marked for deletion at a particular recursion layer of the algorithm. They contain an $x$-coordinate, a pointer LANDING that points to the point element that corresponds to the start/end of the deletion zone (exclusive), a pointer to another divider WRAPPER, integer flags LRANK, RRANK, LAYER, UPDATING, and a bit flag indicating whether the divider is a "left" divider (delete points to the right of this divider) or a "right" divider (delete points to the left of this divider). All of these are initialized to 0 or NULL except for LRANK and RRANK which are initialized to 1.

\textbf{Tangents} represent an upper common tangent between the upper hulls of two subsections. An upper common tangent between two hulls is the line that lies above all points in each hull and which intersects the boundaries of each hull in exactly one contiguous section. This is typically expressed as a pair of extreme points which are the typical intersection points. These are used to determine which points would be eliminated if the two hulls were merged together. In our representation, each tangent simply contains 2 pointers to points, one for the point of tangency of the leftward of the two hulls, LEFTPT, and one for the point of tangency of the rightward of the two hulls, RIGHTPT. Both pointers are set to NULL to start.

The algorithm will utilize four arrays of these types, 2 permanent arrays (of points, $A$, and of dividers $D$) and 2 temporary arrays specific to the particular recursions (of tangents, $T$, and of dividers, $D'$).

\subsection{Marking points for deletion}

Typically, deleting items from an array entails shifting elements later in the array to overwrite them. This can be done in parallel for any number of deletions with $O(n/B)$ cache misses by using a prefix sum to determine the rank of the elements that are not meant for deletion and simply rewriting accordingly. If we do this at every recursion layer of the divide and conquer, this will incur $O(n/B \log \log n)$ cache misses, which would dominate the rest of the algorithm. To avoid this, we will delay deleting points until the very end so that the cost of deletion is only incurred once. We will mark points for deletion during the recursions, taking care to make sure that each point can only be marked once throughout the entire runtime. To achieve this, we will use a permanent divider array, $D$, to store all dividers used across all recursion layers. 
    
\begin{figure}[ht]
    \centering
    \includegraphics[width=.4\textwidth]{images/presorted pointers.png}
    \caption{Showing how the divider array marks points for deletion. Right dividers are solid green squares, left dividers are hollow red squares, and solid black circles are the input points. In orange are the constant length paths taken from marked points to the nearest unmarked point.}
    \label{fig:presortedpoint}
\end{figure}

We use $D$ to keep track of all dividers formed by the descendents of a particular subproblem for two reasons: to identify which points have already been marked for deletion and to form a "highway" from marked points to the nearest unmarked points on their left and right. However, naively this poses an issue for finding the upper common tangents using Overmars and Van Leuwen's \cite{OVERMARS1981166} algorithm since conducting a binary search on an array with some elements marked for deletion could result in landing on a point which has been marked. When a point has been marked, we describe a process for "getting out of the pit", via the dividers.

\begin{algorithm}
\small
\caption{Cache-Optimal algorithm for Presorted Points}\label{alg:presorted}
\KwData{$A$, a subset of points that are sorted by their $x$-coordinate, $n$ the number of points in $A$, $N$ the number of points in the original input, which is a superset of $A$, $E$ an allotted section of global array $D$, $n_E$ the size of alloted section $E$}
\KwResult{The upper hull of $A$}
    \textbf{if $n < \log N$ then} solve using a serial algorithm (such as Graham scan) \;
    \Else{
  Split $A$ into $n^{1/5}$ subproblems of size roughly $n^{4/5}$. Allot a contiguous segment of $\frac{n_E - 2n^{1/5}}{n^{1/5}}$ slots of $E$ to each subproblem (in x-order). Solve these recursively\; 
    Find the common tangents between each pair of subproblems  using the modified Overmars and Van Leuwen technique (See Lemma \ref{lemma:overmars}). Store in a local array of tangents, $T$ \;
       Comparing the elements of $T$ for each subproblem, determine the local set of new dividers, $D'$. Additionally store the dividers in the $2n^{1/5}$ slots at the end of $E$ and another copy in $D'$\;
    Merge the list of old and new dividers by x-order in $E$\;
     For each divider in $E$, update its WRAPPER pointer to the nearest divider which points to a still viable point with its LANDING  pointer, null if it is viable itself\;
   Determine which intervals have points that need to be marked for deletion using the LAYER flags of the dividers on either side. Mark these points accordingly \;
    \textbf{if $n=N$ then} Use prefix sums to determine the ranks of the unmarked (extreme) points and delete the marked points\;
    }
    
\end{algorithm}

\begin{lemma}\label{lemma:pointlookup}
For any point in $A$, the nearest point to the left or right which has not been marked for deletion can be found in $O(1)$ time serially using the permanent divider array, $D$.
\end{lemma}

To determine if a point has been marked for deletion, simply see if its LEFTPAR or RIGHTPAR pointer is anything other than NULL. If so, it has been and we will have to find either the nearest unmarked point to the right or the left, going in the direction away from the previous query on this particular subsection hull. Referring to Figure \ref{fig:presortedpoint}, if we are looking to the nearest to the left, we would follow the orange path from the marked point up to the divider array using the LEFTPAR pointer. After following this pointer, we have gotten to a divider which faces the same direction as we are going (deletes points in the opposite direction). If this divider has a value of NULL for its WRAPPER pointer, then simply follow its POINT pointer, this is the nearest unmarked point. However, if the WRAPPER points to another divider, follow this pointer. This divider will have a WRAPPER pointer value of NULL, so we simply follow its POINT pointer and again have reached the nearest unmarked point.

This rests on maintaining an invariant across runtime: all dividers either point to the nearest point in the appropriate direction (to the left for LEFT and to the right for RIGHT) that hasn't been marked for deletion yet or they point to a divider which points to such a nearest point. The first is clearly true of all new dividers created at a particular recursion layer, since they must point to the point that was the beginning or end of a remaining section of a subproblem. The second requires that we update old dividers that have been made "defunct" by another divider "wrapping" it. For example a LEFT divider with a newer left divider to its immediate left. The "defunct" LEFT divider will point, via its wrapper flag to the nearest LEFT divider which has not yet been made defunct.

\begin{lemma}\label{lemma:overmars}
For any two hulls of size $\leq n^{4/5}$, their upper common tangent can be found in $O(\log n)$ time serially using the point array $A$.
\end{lemma}

This follows from Lemma \ref{lemma:pointlookup}, since a simple adjustment to Overmars and Van Leuwen's \cite{OVERMARS1981166} algorithm where queries for points also include the relative position of the previous query on that hull suffices to accomplish this. So, if we came from a point that is to the left of where we start the query, we want to find the nearest unmarked point to its right (or itself if it's unmarked). This is to prevent an infinite loop where the same point is considered multiple times. When moving away from the previous, the point query is always able to eliminate half of the points in contention if this can be done in the standard procedure. Consider the point that was initially queried as $p$ and the point, $p'$, that it lands on after following the chain and \textit{wlog} considering $p'$ to be to the right of $p$. If the comparison resulting from the query tells us that the point of tangency must be to the left of $p'$, it must also be to the left of $p$ since $p$ is unmarked. If the comparison tells us that the point of tangency must be to the right of $p'$, then everything to the left of $p'$ including everything to the left of $p$ is removed from consideration. Therefore, since the search space is cut in half or even more, the same binary search procedure from Overmars and Van Leuwen works with this slight adjustment.

\begin{lemma} \label{lemma:newdividers}
The set of new dividers, $D'$, for a particular recursion layer can be found in $O(n^{2/5} \log n)$ work and $O(\log n)$ span.
\end{lemma}

To find the set of new dividers, we start by finding the common tangents between every pair of hulls as in Atallah and Goodrich \cite{ATALLAH1986}. From Lemma \ref{lemma:overmars}, we can do this in parallel for all $\binom{n^{1/5}}{2}$ pairs of hulls in $O(n^{2/5} \log n)$ work and $O(\log n)$ span. We store these tangents in a local array, $T$, so that for every subproblem hull there are $n^{1/5}-1$ tangents that relate to it. From there, we look in parallel at each hull's tangents to find which has the smallest and which has the largest slope. If these slopes indicate that the points of this hull lie below both of these lines of tangency, then those points will be marked for deletion since they are clearly inside the hull. Otherwise, we take the sequence of points between the point of tangency for the tangent with smallest slope and the point of tangency for the tangent with largest slope as the surviving points from this recursion layer.

At the leftmost end of the surviving sequence of points for a particular hull, we place a RIGHT divider, indicating that deletion stops at this point. Here, placing a divider $d$, at a point $p$ means declaring $d$ to have the same x-position as $p$ and $d$'s LANDING pointer to point to $p$. We place a LEFT divider at the rightmost point of the remaining section. This indicates that point deletion should resume going rightwards. It is known that the point with the smallest x-coordinate in a set of points are points on the hull. So, for the leftmost hull, the surviving sequence will include the leftmost point, indicating that there is no need for a LEFT divider all the way to the left indicating to start deletion. For hulls that have no points to contribute, we don't need to include any dividers at all.



 Therefore, to find the entirety of $D'$ is dominated by the work to find the common tangents, $O(n^{2/5} \log n)$.


\begin{theorem} \label{lemma:deletionmark}
When applying Algorithm \ref{alg:presorted} to a set of $n$ points, marking points for deletion incurs $O(n/B)$ cache misses and $O(n)$ work total. 
\end{theorem}

After finding the $\leq 2n^{1/5}$ new dividers, which are in x-sorted order by the subproblem partition, we will incorporate them with the dividers used in lower layers of the recursion. Since we keep the list of these dividers separate and in x-sorted order (each of the subproblems have their dividers sorted and the subproblems themselves are sorted by x) we can simply combine the new dividers with the old ones using a list merging algorithm. Each divider has two copies, one in $D$ and one in $D'$, and we will be storing a pointer to the $D$ copy in the $D'$ copy once the sorting is done. The merging of the new and old dividers in $D$ can be done using Blelloch and Gibbons' \cite{BlellcohGibbons} algorithm which incurs $O(n/B)$ cache misses, or in this case $O(\frac{n}{B \log n})$ since the total size of $D$ is $\frac{4 n}{\log n}$. In case there are gaps in the list of the old dividers due to there being fewer dividers produced than expected in some subproblems, we can find the ranks of the nonempty dividers and condense the lists into one by using a prefix sum, incurring same cost in terms of work, span and cache misses as the later merge.

Once the dividers are sorted, we can determine which sections need to be deleted. Within the part of $D$ available to this subproblem, check all sections of $A$ with a LEFT divider on its left end and a RIGHT divider on its right end. In other word, check intervals between dividers with indices of the form $2k+1$ and $2k+2$ for $k>0$ (with 0 being the first index in the alloted section of $D$). If one of the boundaries of this is a new divider, then mark the points in $A$ corresponding to the interval to be deleted. If one of the dividers is old, mark the endpoint pointed to by the old divider, since this was not previously marked. Marking a point for deletion is done by setting the LEFTPAR pointer to the nearest LEFT divider and RIGHTPAR to the near RIGHT divider. For any interval, say of size $I$, the total number of cache misses incurred is equal to $\lceil I /B \rceil \leq \lfloor I/B \rfloor +1$, of which we can charge the 1 to the number of new dividers to add $O(n^{1/5})$ misses to this layer and the rest will be charged to the running total for markings, $O(n/B)$ since each point will be marked at most once.

After marking these, we will have to update the "highway". The deprecated dividers need to now point to the nearest divider, to their left if it's a LEFT divider and to the right if it's a RIGHT divider. These updates are only done on those dividers which are to the right of a LEFT divider and to the left of the corresponding RIGHT divider. Those dividers which require updating can be identified with a series of prefix sums. Using the LAYER flag, we have stored what layer of the recursion this divider originated from (set this during the creation of new dividers). Using a prefix sum that counts new dividers that are left dividers as 1s and right dividers as -1s. Storing this information in the UPDATING flag, we can determine whether a divider is between two new dividers. Since we start with a right divider, all dividers which need updating will have an UPDATING value of 0 and all those which do not will have an UPDATING value of -1 after the prefix sum. From here, we determine the number of new LEFT dividers to its left using another prefix sum stored in LRANK and going the reverse direction the number of new RIGHT dividers to the right, stored in RRANK. This allows us to determine for the updating divider which new divider needs to be linked to in the WRAPPER pointer. 

First, we need to make sure that the elements of $D'$ point to their copies, using a binary search. This will incur $O(n^{1/5} \log n)$ cache misses, which is dominated by $O(\frac{n}{B \log n})$. For LEFT dividers, the LRANK indicates the rank in $D'$ that corresponds to the "wrapping" divider that it will point to on the highway. For RIGHT dividers, RRANK indicates the same but counting from the opposite end of the array. So we can simply copy the WRAPPER pointer from the appropriate $D'$ element for all dividers in $D$ with UPDATING set to 0 (as opposed to -1). Any new dividers must instead have WRAPPER set to NULL, since they will also have UPDATING set to 0. Once these are set, the highway is maintained, allowing for efficient search using the modified Overmars procedure. The total work incurred for these operations on $D$ is $O(\frac{n}{B \log n})$, meaning the entire procedure of marking for deletion incurs at most $O(n/B)$ cache misses across all recursion layers.

\subsection{Cache, Work and Span Analysis}

\begin{lemma} \label{lemma:postdeletioncost}
Once all non-extreme points have been marked for deletion, the convex hull can be given as a sorted array of points in $O(n/B)$ cache misses, $O(n)$ work and $O(\log n)$ span.
\end{lemma}

Removing all the points that have been marked for deletion  can be done afterwards by simply computing the ranks of the unmarked points in the final array using a prefix sum. After this, we can use the calculated ranks to move all of the surviving points to contiguous locations at the beginning of $A$, updating the size of the array accordingly. This prefix sum is done using $O(n/B)$ cache misses, $O(n)$ work and $O(\log n)$ span, so we stay within our desired bounds. Simply 

\begin{theorem}
Applying Algorithm 1 to a set of $n$ points incurs $O(n/B)$ cache misses, $O(n)$ work and $O(\log n)$ span.
\end{theorem}

From Lemma \ref{lemma:postdeletioncost}, we know that once the points are marked for deletion, only an additional $O(n/B)$ cache misses, $O(n)$ work and $O(\log n)$ span are incurred. We know from Lemma \ref{lemma:deletionmark} that the total cost of marking points for deletion across all recursion layers amortizes to $O(n/B)$ cache misses, $O(n)$ work and contributes only $O(\log n)$ span. From here, the remaining work relates to the work done at each layer. This work is dominated by the merge operation used on the permanent list of dividers, $D$. At each layer, the total amount of work due to this merge is $O(\frac{n}{\log n})$ since the total size of the array is bounded by a constant times the number of subproblems that use the base case algorithm, which is $n/\log n$. This follows from the fact that each recursion layer splits into at least twice as many subproblems as the previous, so the number leaves of a rooted tree to represent this recursion is at least half the total number of nodes. This work, done across $\log \log n$ recursion layers is equal to $O(\frac{n \log \log n}{\log n})$ which is dominated by the $O(n)$ work from marking points for deletion. 

The cache misses at each recursion layer of size $r$ follows similarly, $O(\frac{r}{B \log r})$, but special care is taken to make sure that the total cache misses from the binary searches, $O(r^{2/5} \log r)$, does not exceed $O(n/B)$ when summed across lower recursion layers. These additional cache misses are incurred until the subproblems size is $M$ or $\log n$, whichever is larger. In either case, this will be larger than $B^2$ since we are using a tall cache assumption ie. $M = \Omega (B^2)$. Observe that for any particular recursion layer with $r$ points remaining, the number of misses from this layer is $O(r^{2/5} \log r)$ and the total number from all of its subproblems is $O(r^{1/5} \cdot (r^{4/5})^{2/5} \log (r^{4/5})) = O(r^{13/25} \log r)$. This implies that the complexity of these additional cache misses increases asymptotically as we descend to deeper recursions. The final layer before a subproblem of size $M$ is a subproblem of size $M^{5/4}$. This layer will incur $O(\frac{n}{M^{5/4}} \cdot (M^{5/4})^{2/5} \log (M^{5/4}) = O(\frac{n\log M}{M^{3/4}})$ cache misses . Since $O(\log M) \subset O(M^{1/4})$ and $M \subset \Omega (B^2)$, this is clearly $O(\frac{n}{M^{1/2}}) \subset O(\frac{n}{B})$. The same logic applies if the final layer is of size $\log n$. Therefore, the cache misses are $O(n/B)$ in total.

At each recursion layer, we incur $O(\log n)$ span. The subproblems can be done in parallel, giving us a recurrence of $T_\infty (n) = T_\infty (n^{4/5}) + O(\log n)$ which solves to $O(\log n)$. So, the total span is $O(\log n)$. This means that Algorithm 1 runs in $O(\log n)$ span with $O(n)$ work and $O(n/B)$ cache misses. 


\subsection{Additional Cache Misses from Work-Stealing and False Sharing}

\begin{theorem}
Algorithm \ref{alg:presorted} incurs $O(\frac{n}{B} + S \cdot \frac{M}{B})$ cache misses (including false shares) under a work-stealing scheduler, where $S$ is the number of steals.
\end{theorem}

In the previous discussion of the number of cache misses incurred across the runtime of the algorithm, the only remaining source of cache misses is the scheduler. We use the same notion of work stealing as in Cole and Ramachandran \cite{ColeRamachandran}, ie that in parallel sections, each processor places tasks into a work queue, and where idle processors "steal" work from the tops of these queues to decrease runtime. Associated with work-stealing is an additional type of cache misses, known as false sharing. False sharing occurs in private cache settings when a processor $P_1$ writes to a block which had previously been stored in the cache of another processor $P_2$ and then $P_2$ now has to access that block. Each step in Algorithm \ref{alg:presorted} corresponds to a set of parallel tasks, with synchronization after the conclusion of each step to ensure correctness. There is only one step in which different tasks share any data, (Step 5) however concurrently reading from the same locations do not incur any false shares. However, false shares can result from data alignment. 

For cache-oblivious algorithms, there is no guarantee that subproblems will be partitioned along block boundaries. This can incur at most 1 additional cache miss per boundary due to false sharing. If we implement each step recursively, then we can ensure that these boundaries will only contribute a constant factor of additional false shares before steals. This applies to all steps, 4 through 9, but is redundant for step 6 as Blelloch and Gibbons \cite{BlellcohGibbons} is already implemented recursively. 

Steals are another source of false shares. All of our steps 4 through 9 write to singular, contiguous array locations within each parallel task. Tasks are ordinarily distributed to processors such that the write locations for successive tasks will be contiguous to each other. However, this contiguity can be disrupted by a steal. Even though a thief may update a piece of memory that won't be needed by the original processor, it may be within a block that is within the original processor's private cache, incurring a false share.  Any particular write can affect at most $B-1$ other processors which are operating in the same area, meaning that false shares only contribute $O(S \cdot B) \subset O(S \cdot \frac{M}{B})$ additional cache misses.

Aside from false shares, the only additional cache misses incurred due to steals are those incurred due the stealing processors accessing data that ordinarily would have been accessed by the original processor in order. This could be as bad as a stealing processor completely reloading as many blocks as could fit into the cache, implying at worst $O(S \cdot \frac{M}{B})$ cache misses. So in total, when using any work-stealing scheduler, there is at most $O(\frac{n}{B} + S \cdot \frac{M}{B})$ cache misses incurred by Algorithm \ref{alg:presorted}.

\begin{corollary}
Algorithm \ref{alg:presorted} incurs $O(n/B)$ cache misses \textit{w.h.p} in $p$ with the RWS scheduler when the number of processors is $p = O(\frac{n}{M \log n})$. 
\end{corollary}

We additionally consider a randomized work-stealing scheduler, the same as is described in Cole and Ramachandran \cite{ColeRamachandran} and which was originally described by Blumofe and Leiserson \cite{BlumodeLeiserson}. The randomized work-stealing scheduler (RWS) is a work-stealing scheduler where "idle" processors steal the head task from a randomly selected processor. If this fails, as in the task queue selected is empty, the scheduler simply tries again until either a task is found or the parallel section is completed.

Acar, Blelloch, and Blumofe \cite{acar2000data} show that w.h.p. in $p$, the number of steals incurred during execution using the RWS is $S = O(p \cdot T_\infty)$. Therefore, if $p = O(\frac{n}{M \log n})$, then $S = O(\frac{n}{M})$, which when applied to the total number of cache misses yields $O(\frac{n}{B} + \frac{n}{M} \cdot \frac{M}{B}) = O(n/B)$.

==> algorithm_docs/presortedalt.tex <==
\section{A Cache-Optimal \texorpdfstring{$O(\log n)$}{O(log n)} Span Algorithm for Presorted Points}

We present a cache-oblivious divide-and-conquer algorithm for finding the upper convex hull of an array of presorted points. It achieves $O(\log n)$ span with $O(n)$ work and $O(n/B)$ cache misses, which are optimal bounds for work, span, and cache efficiency for the convex hull problem in the binary-forking model. As is common practice, we describe a procedure which finds the "upper hull", the set of extreme points which lie above the line from the leftmost and rightmost points. Repeating this procedure on the point set rotated by 180 degrees yields the entire convex hull. We consider our algorithm to be one of several to build off of the recursive structure of Atallah and Goodrich's \cite{ATALLAH1986} $O(n \log n)$ work algorithm. Atallah and Goodrich's algorithm is a $\sqrt{n}$-way divide-and-conquer algorithm. To perform the merges, it uses Overmars and Van Leuwen's \cite{OVERMARS1981166} technique for finding the upper common tangent of two disjoint convex polygons to compare the $\sqrt{n}$ subproblem solutions and determine which points from each should remain. At each layer in this recursion, $\binom{\sqrt{n}}{2} = O(n)$ applications of this technique are used at the cost of $O(\log n)$, giving the recurrence $T(n) = \sqrt{n} T(\sqrt{n}) + O(n \log n)$ for the total work. The span of this method is $O(\log n)$, even under the more restrictive binary-forking model where $O(\log n)$ is optimal for any problem requiring $\Omega(n)$ work, as spawning $\Omega(n)$ threads incurs $\Omega(\log n)$ span. However, here the work remains suboptimal.

Goodrich \cite{goodrich1987finding} presented a method to obtain $O(n)$ work using a tree data structure which they refer to as a ``hull tree''. The hull tree data structure stores the convex hull of a set of points in a binary tree that permits a simulation of the Overmars and Van Leuwen's procedure and an efficient means of ``trimming off'' points that have been eliminated and unifying subproblem solutions under a new tree. The issue is that using this data structure incurs many cache misses because the tree cannot guarantee any data locality. Chen \cite{chen1995efficient} also uses a tree-based approach to achieve $O(n)$ work, which encounters the same issue.

The first step to ensure data locality while reducing to $O(n)$ work is to decrease the number of subproblems so that the pairwise hull comparisons do not take $O(n \log n)$ work. In fact, we want this work from these comparisons to total $O(n/B)$. This can be done by choosing a different exponent. We will use $n^{1/6}$-way divide-and-conquer, which means that comparing the subproblem solutions will take $O(n^{2/6} \log n)$ work, which allows us to use the tall cache assumption ($M = \Omega(B^2)$) to bound the total work from these comparisons by $O(n/B)$. Once the subproblems are compared, we can eliminate all of the points which have been determined to be within the hull by shifting all of the remaining points to the front of the array (using a prefix sum). This can be done cache-obliviously \cite{blelloch2010low}, incurring $O(n/B)$ cache misses for each recursion layer. However, this comes out to be $O(n \log \log n)$ work total. So, if we are to maintain data locality, we have to determine a way to eliminate points without having to shift everything down and incur too much work.

Instead of deleting points immediately, Algorithm \ref{alg:presorted}, (pseudocode in appendix) uses an array of size $O(\frac{n}{\log n})$ which stores a set of x-coordinate intervals corresponding to the points which must be deleted. We store these intervals as a list of ``starts'' and ``ends'' which correspond to the beginning and ending of each deletion interval all sorted by x-coordinate. For an interval $I$, consider the largest interval $I'$ for which $I \subseteq I'$. As an invariant, we will store in $start(I)$ a pointer to $start(I')$ and in $end(I)$ a pointer to $end(I')$. This will crucially allow us to get from a point that is within one of these intervals to the nearest point which is not within any of these deletion intervals in $O(1)$ time, which lets us simulate the Overmars and Van Leuwen \cite{OVERMARS1981166} technique on subproblem solutions. By primarily operating on this array of intervals, we can avoid incurring $O(n)$ work at every layer and instead amortize to $O(n)$ total work across all layers.


\subsection{Data Structure Invariants}

We use three data types in our arrays: \textbf{points}, \textbf{dividers}, and \textbf{tangents}. Each type is constant-sized, so the arrays have space linear in their respective numbers of elements.

\textbf{Points} are based on the input, with some extra attributes assigned to each point so that if it is not an extreme point, it can be marked instead of immediately removed. In addition to $x$- and $y$-coordinates, the point contains a \textrm{\sc{\em{Rank}}} integer flag which is initialized to 1 and two pointers to dividers called $\textrm{\sc{\em{LeftPar}}}$ and \textrm{\sc{\em{RightPar}}}. $\textrm{\sc{\em{LeftPar}}}$ and \textrm{\sc{\em{RightPar}}} are initialized to \textrm{\sc{\em{Null}}}, but when they are set, they indicate that the point is within some deletion interval $I$. $\textrm{\sc{\em{LeftPar}}}$ points to a divider corresponding to the start of $I$, whereas \textrm{\sc{\em{RightPar}}} points to a divider corresponding to the end of $I$.


\textbf{Dividers} represent the \textit{boundaries} of deletion intervals. If the divider represents the beginning of some interval $I$, we will refer to it as $L_I$. If the divider refers to the end of $I$, then we will refer to it as $R_I$. The divider contains an $x$-coordinate, a pointer \textrm{\sc{\em{Landing}}} that points to the point element  corresponding to the start/end of the interval (but not within the interval), a pointer \textrm{\sc{\em{Wrapper}}} to a divider from an interval $I'$ that is a superset of $I$ ($L_I'$ for $L_I$ and $R_I'$ for $R_I$), an integer flag \textrm{\sc{\em{Rank}}} for use in prefix sums, a bit flag  \textrm{\sc{\em{Marked}}} to denote whether  \textrm{\sc{\em{Landing}}} has been marked, and a bit flag indicating whether the divider is a ``\textrm{\sc{\em{Left}}}'' divider (the start of an interval) or a ``\textrm{\sc{\em{Right}}}'' divider (the end of an interval). All of these are initialized to 0 or \textrm{\sc{\em{Null}}}.

\textbf{Tangents} represent an upper common tangent between the upper hulls of two subsections. An upper common tangent between two hulls is the line that lies above all points in each hull and which intersects the boundaries of each hull in exactly one contiguous section. This is typically expressed as a pair of extreme points, one from each hull. These are used to determine which points would be deleted if the two hulls were merged together. In our representation, each tangent simply contains 2 pointers to points, one for the point of tangency of the leftward of the two hulls, and one for the point of tangency of the rightward of the two hulls. Both pointers are set to \textrm{\sc{\em{Null}}} to start.

Our presorted algorithm will utilize 4 arrays of these types: 2 permanent arrays (of points, $A$, and of dividers $D$) and 2 temporary arrays specific to the particular recursions (of tangents, $T$, and of dividers, $D_{new}$).

There are 5 invariants that are maintained with respect to $D$ that will allow us to bound our work by $O(n)$ and our cache misses by $O(n/B)$.

\begin{enumerate}[align=left,label=\textbf{Invariant \arabic*},ref=\arabic*]\setlength{\itemindent}{.35cm}
    \item \label{invariant:1} The size of $D$ must be $O(\frac{n}{\log n})$.
    \item \label{invariant:2} For any interval $I$ with dividers $L_I, R_I \in D$, and the largest subset $I'$ such that $I \subseteq I'$, $L_{I}.\textrm{\sc{\em{Wrapper}}}= L_{I'}$ and $R_{I}.\textrm{\sc{\em{Wrapper}}}= R_{I'}$. In the case of ties, take $I'$ to be that was most recently added.
    \item \label{invariant:3} For any two intervals $I_1,I_2$ with dividers in $D$, either $I_1 \cap I_2 = \emptyset$, $I_1 \subseteq I_2$, or $I_2 \subseteq I_1$.
    \item \label{invariant:4} For any point $p$ which is in at least one interval, for one such interval $I$, $p.\textrm{\sc{\em{LeftPar}}} = L_I$ and $p.\textrm{\sc{\em{RightPar}}} = R_I$. 
    \item \label{invariant:5} For any interval $I$ for which $L_I.\textrm{\sc{\em{Wrapper}}} = L_I$ and $R_I.\textrm{\sc{\em{Wrapper}}} = R_I$, then neither $L_I.\textrm{\sc{\em{Landing}}}$ nor $R_I.\textrm{\sc{\em{Landing}}}$ are elements of any interval.
\end{enumerate}

\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[height=.5\textwidth]{images/interval traversal.png}
        \caption{}
        \label{fig:intervaltraversal}
    \end{subfigure}
    \begin{subfigure}[b]{0.65\textwidth}
        \centering
        \includegraphics[height=.5\textwidth]{images/overmars simulation.png}
        \caption{}
        \label{fig:overmarssim}
    \end{subfigure}
    \caption{(a) Example of paths from marked points to points that have not been marked; (b) Simulating the Overmars and Van Leuwen \cite{OVERMARS1981166} procedure using the divider array. Only one of the two hulls are depicted. The blue line depicts the current point of consideration and the green the previous point of consideration.}
    \label{fig:my_label}
\end{figure}

We give an example depiction of this structure in Figure~\ref{fig:intervaltraversal}. We show this in the context of paths from points that are marked for deletion (lie in some interval) to a nearest point to the left or right which is not in that interval. Assuming the invariants hold, we can claim the following theorem.

\begin{theorem}\label{thm:overmars}
    Given two convex hulls $C_1$, $C_2$, that are both expressed by an array of points $A$ and an array of dividers $D$, and that are separable by a vertical line, the upper common tangent of $C_1$ and $C_2$ can be computed in $O(\log n)$ time serially.
\end{theorem}

\begin{proof}
We give a full proof of this in Section \ref{sec:fullovermars}. The procedure is very similar to the original Overmars and Van Leuwen routine \cite{OVERMARS1981166}, but with special care being taken to deal with the case in which the binary searches land inside an interval. This is a possibility since the array is composed of both extreme points and points which we already know are not. In short, we can "dig ourselves out" whenever this happens by considering both the nearest extreme point to the left and the nearest extreme point to the right of the non-extreme point. We do so by taking advantage of the 5 invariants above, particularly invariants \ref{invariant:2}, \ref{invariant:4}, and \ref{invariant:5} to find constant length paths to these points. These constant length paths allow the runtime of a particular comparison to be simply $O(\log n)$, incurring only a constant factor over the original. \end{proof}


\subsection{Maintaining the invariants}

Now that we have a method to compare the hulls assuming the invariants hold, we will show how to merge the hulls, keeping in mind that we also must maintain the invariants. Lemma \ref{lma:dividercreation} will show how to maintain invariants \ref{invariant:1} and \ref{invariant:3}, while Lemma \ref{lma:markingpoints} will show how to maintain invariants \ref{invariant:2}, \ref{invariant:4}, and \ref{invariant:5}.

\begin{lemma} \label{lma:dividercreation}
The set of new dividers $D_{new}$ for a given recursion layer (of size $n$) can be determined in $O(\log n)$ span with $O(n^{2/6} \log n)$ work (and cache misses)
\end{lemma}
\begin{proof}
We will first calculate the $O(n^{2/6})$ common tangents, storing them in a 2D array $T$. We use the smallest and largest sloped tangents (as in Atallah and Goodrich \cite{ATALLAH1986}) to determine which points should be removed from each subproblem hull, or subhull. For each subhull, there will be some section starting with the leftmost point and some section starting with the rightmost point which will need to be removed, leaving some contiguous set of points in the center, or no points from this hull. If there is such an set, we use a \textrm{\sc{\em{Right}}} divider with \textrm{\sc{\em{Landing}}} set to the first (leftmost) unremovable point and a \textrm{\sc{\em{Left}}} divider with \textrm{\sc{\em{Landing}}} set to the last (rightmost) unremovable point. If there are no unremovable points from this subhull, then do not add any divider. We can omit dividers for the leftmost and rightmost points among all of these subhulls, since they will not correspond to intervals of deletion (they are extreme points). We can store these all in an array of size $2n^{1/6}-2$, with gaps allowed for nonexisting dividers. Set the \textrm{\sc{\em{Wrapper}}} for each of these dividers to itself.

At this point, $D_{new} \cup D$ has satisfied invariants \ref{invariant:1} and \ref{invariant:3}. \ref{invariant:1} is satified since $D$ must be of size at most $O(\frac{n}{5/6 \log n})$ and the addition of $2n^{1/6}-2$ dividers does not affect this asymptotically. \ref{invariant:3} is satisfied by induction, since when $D$ is empty, this holds since it holds for $D_{new}$ alone, and assuming it holds for $D \neq \emptyset$, since $D_{new}$ does not have dividers that "land" inside previously marked points, they cannot intersect with any previous intervals corresponding to $D$ without entirely containing such an interval.
\end{proof}

\begin{lemma}\label{lma:dividerintegration}
The set of new dividers $D_{new}$ for a given recursion layer (of size $n$) can be integrated into the full set of dividers $D$ in $O(\log n)$ span with $O(\frac{n}{\log n})$ work and $O(\frac{n}{B \log n})$ cache misses.
\end{lemma}
\begin{proof}
We can integrate these using a merge routine. Specifically, we will be merging a copy of $D_{new}$ into $D_{alloted}$, a set of contiguous slots in $D$ that have been allotted to this subproblem. After alloting for each of the subproblems, there are $2n^{1/6}$ slots remaining at the end, allowing us to copy $D_{new}$ there. Before doing so, we will compress $D_{new}$ so they occupy contiguous positions. Only then will we copy them over to the end of $D_{alloted}$. These both can be done using prefix sums \cite{blelloch2010low}, which takes $O(n^{1/6})$ work and $O(n^{1/6}/B)$ cache misses. These calculations will use the \textrm{\sc{\em{Rank}}} flag. \end{proof}

\begin{lemma} \label{lma:markingpoints}
All non-extreme points can be marked for deletion with $O(n)$ work and $O(n/B)$ cache misses, amortized.
\end{lemma}
\begin{proof}

We show that every cache miss incurred by the process of marking points for deletion can be charged either to the binary searches (which we show to be $O(n/B)$ in Theorem \ref{thm:presorted_final}) or to the total number of blocks representing the points. We also show that the remaining invariants hold. 

%Issue: We may need to mark points in some 

Now that the array $D_{new}$ has copies of its elements integrated into $D_{alloted}$, we can start by satisfying invariant \ref{invariant:2}. For each adjacent pair in $D_{new}$ corresponding to an interval of deletion $I$, conduct binary searches on $D_{alloted}$ for their copies. Between these two copies will be a set of dividers corresponding to intervals which are subsets of $I$. We have already marked the points inside these intervals, so we just need to mark what is left. We start with the points between the beginning of $I$ and its first subset, and the points between the last subset and the end of $I$. To determine these subsets, we will store the rank in $D_{alloted}$ of the copies in the \textrm{\sc{\em{Rank}}} flags of the $D_{new}$ elements. For the ``in-between'' dividers in $D_{alloted}$ which are \textrm{\sc{\em{Left}}}, set their \textrm{\sc{\em{Wrapper}}} pointers to the \textrm{\sc{\em{Left}}} element of the $D_{new}$ pair, specifically the copy in $D_{alloted}$. For the \textrm{\sc{\em{Right}}} divider, do the same with the \textrm{\sc{\em{Right}}} copy. This will satisfy invariant \ref{invariant:2} by the same principle of induction as before.  All that remains is to mark the points inbetween subintervals of $I$. These points are distinguished by being between dividers which have their  \textrm{\sc{\em{Marked}}} flag set to false (the default) and which are themselves between a \textrm{\sc{\em{Left}}}-\textrm{\sc{\em{Right}}}divider pair from $D_{new}$. We will set each point's \textrm{\sc{\em{LeftPar}}} to the left divider of the subinterval after the point and the \textrm{\sc{\em{RightPar}}} to the right divider of the subinterval before the point. This will still let the point reach to the nearest unmarked point, since the subintervals all point to the largest superset.

The marking procedure is cache efficient, incurring $O(\frac{n}{B \log n})$ cache misses at each recursion layer. There can be additional cache misses incurred due to the deletion marking intervals not aligning with blocks, but these misalignments can only happen at the edges of the interval, which means we can charge 2 cache misses to one of the binary searches used to compute that divider earlier. The searches are not cache efficient, but only incur $O(n^{1/6} \log n)$ work, which is dominated by the binary searches used for comparing the subhulls, which are analyzed in Theorem~\ref{thm:presorted_final}.

At this point, invariant \ref{invariant:5} has already been satisfied. Now that the \textrm{\sc{\em{Wrapper}}} flags have been set for intervals that are subsets, we can note that from before the \textrm{\sc{\em{Landing}}} flags for $D_{new}$ elements will not land inside previously marked points. This means that the only way a divider $d$ could have a \textrm{\sc{\em{Landing}}} which has been marked for deletion is if that landing were in a new interval, in which case the interval of $d$, $I$, is a subset of the interval that marked $d.\textrm{\sc{\em{Landing}}}$, by \ref{invariant:3}.

All that remains is invariant \ref{invariant:4}. To maintain this, we mark the points for deletion. To ensure that we do not mark twice, we only consider intervals that were previously unmarked in the previous iteration, or those that are between dividers from $D_{new}$.  Consider a divider $d\in D_{new}$ Let $d'$ be the corresponding divider to $d$ that together represent interval $I$. Looking at the copy of $d$  in $D_{alloted}$, we take the neighboring divider: $D_{alloted}[d.\textrm{\sc{\em{Rank}}}+1]$ if $d$ is a \textrm{\sc{\em{Left}}} divider and $D_{alloted}[d.\textrm{\sc{\em{Rank}}}-1]$ if $d$ is a \textrm{\sc{\em{Right}}} divider. These dividers have landing spots, between which are points will be marked for deletion (exclude the landing spot of a $D_{new}$). Consider the $d$ to be \textrm{\sc{\em{Left}}}. Set $\textrm{\sc{\em{LeftPar}}}$ to $D_{alloted}[d.\textrm{\sc{\em{Rank}}}]$ and \textrm{\sc{\em{RightPar}}} to $D_{alloted}[d'.\textrm{\sc{\em{Rank}}}]$. Do the reverse if $d$ is \textrm{\sc{\em{Right}}}. This will satisfy invariant \ref{invariant:4}. We will mark the points in parallel, in groups of size at most $\log n$.

\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth]{images/deletion_marking.png}
    \caption{Each pair in $D_{new}$ binary searches for its copy, marks its subsidiaries and then marks the "outermost layer" of points.}
    \label{fig:deletionmarking}
\end{figure}

Since only points in "new" intervals are marked, this means that each point is marked at most 1 time, allowing us to amortize the work of marking to $O(n)$. We address some issues due to data alignment in \ref{sec:cachepresort}, but note here that the marking of points is done to adjacent points. We can charge 2 cache misses from each of these to the elements of $D_{new}$, which allows us ignore the issues of alignment on the ends of these intervals. This allows us to consider the "middles" of these intervals, which are access cache-efficiently. These will amortize to $O(n/B)$.\end{proof}



\subsection{Work, Span, and Cache Analysis}

\begin{theorem}\label{thm:presorted_final}
    Algorithm \ref{alg:presorted} achieves $O(\log n)$ span with $O(n)$ work and incurring $O(n/B)$ cache misses
\end{theorem}

\begin{proof}
First, we show span. To start, Algorithm \ref{alg:presorted} finds the convex hull of $O(\frac{n}{\log n})$ subhulls at the lowest level in the recursion layer. Each individual subhull is done serially using a serial algorithm. The Graham scan\cite{Graham1972AnEA} is ideal since it achieves $O(n/B)$ cache misses for presorted input. With each subhull having size at most $\log n$, this takes $O(\log n)$ span. From here, merges are used. The merges start with finding the new dividers $D_{new}$, which takes $O(\log n)$ span from Lemma \ref{lma:dividercreation}. From there, integrating them into the full set of dividers takes $O(\log n)$ span from Lemma \ref{lma:dividerintegration}. Finally, marking the points for deletion takes $O(\log n)$ span due to the binary searches. Marking the points and old dividers takes no more than $O(\log n)$ span since each point/divider can be done in parallel. This gives us the following recursion which solves to $O(\log n)$:

$$T_\infty(n) \leq T_\infty(n^{1/6}) + c_1 \log n $$

This expands to $c_1 \log n + \frac{c_1 \log n}{5} + . . . $ which is clearly bounded by $2 c_1 \log n = O(\log n)$ The final step, using a prefix sum to align the unmarked points into adjacent array positions, takes only an additional $O(\log n)$ span \cite{blelloch2010low}.

For the work, the total work is dominated by the final prefix sum, $O(n)$ \cite{blelloch2010low}. The $O(\frac{n}{\log n})$ base cases of size $\log n$ cost $O(n)$ work in total when Graham's algorithm is used. From Lemma \ref{lma:markingpoints}, we know that marking points for deletion costs only $O(n)$ work amortized. From here, it suffices to show that all other operations cost $O(\frac{n}{\log n})$ work per recursion layer. The work from Lemmas \ref{lma:dividercreation} and \ref{lma:dividerintegration} are dominated by $O(\frac{n}{\log n})$, which leaves the work on the divider array leading up to point marking. Setting the old dividers' \textrm{\sc{\em{Wrapper}}} flags is linear in the size of $D_{alloted}$, the available section of divider array. This is $O(\frac{n}{\log n})$ where $n$ is the size of this recursion instance. Therefore, for the recursive steps, we have the following recursion for work:
$$T_1'(n) \leq n^{1/6}T_1'(n^{5/6}) + c_1\left(\frac{n}{\log n}\right)$$
Since we accounted for the base cases earlier, we can set $T_1'(\log n) = 0$, We get that total work in $T_1'(n)$ is at most $\frac{c_1 n \log \log n}{\log n}$ which is clearly dominated by $O(n)$. Therefore, $T_1(n) = T_1'(n) + O(n) + O(n) = O(n)$

For cache misses, we know that the serial algorithm on the $O(\log n)$ sized subproblems incurs $O(n/B)$ cache misses. From Lemma \ref{lma:markingpoints}, we know that marking the points can be amortized to $O(n/B)$ by charging inefficiently marked points to the binary searches. The recursive layers are cache efficient with the exception of $O(n^{2/6} \log n)$ binary searches (and other factors dominated by this). The cache efficient routines incur at most the work divided by $B$, which is $O(n/B)$. The binary searches incur misses until the recursion size is $M$ or $\log n$, whichever is greater. If $\log n$ is greater, then simply bounding by the total work done in the recursions suffices, since for sufficiently large $n$ and any positive constant $c$, $c\frac{n \log \log n}{ \log n} \leq c\frac{n \log M}{M}\leq c\frac{n M^{1/2}}{M} = c\frac{n }{M^{1/2}}$ . By tall cache assumption i.e. $M = \Omega(B^2)$, and thus $\frac{1}{M^{1/2}} = O(\frac{1}{B})$ , the cache misses can be bounded by $O(\frac{cn}{B})=O(n/B)$.

If $M > \log n$, then we consider the following recursion:

$$Q(n) \leq n^{1/6} Q(n^{5/6}) + c_1 n^{2/6}\log n$$

We complete the analysis of cache misses in the parallel setting in Section \ref{sec:cachepresort}. \end{proof}



==> algorithm_docs/random.tex <==
\section{A Randomized Algorithm with Optimal Work and Span WHP in $n$}
\label{sec:random}
We also present an adaptation of Ahmad et al.'s \cite{ahmad} randomized sorting algorithm which matches its bounds, $O(\log n)$ span and $O(n \log n)$ work, both \textit{whp} in $n$. It follows mostly the same format as the sorting algorithm. It is comprised of an Almost-Sort algorithm that returns a sorted list of some of the elements and a Full-Sort algorithm that calls on the Almost-Sort and then reincorporates the elements not included in its output.  The Almost-Sort algorithm uses a bucket based approach, first by sorting a sample of $\sqrt{n} \log ^3 n$ elements to form pivots for the buckets and then attempting to place elements into the buckets. If two or more elements try to write to the same slot in the bucket, this is considered a collision and only one of them is written while the others are set aside for processing later. This bucketing is done recursively until they are of size $n^{1/\log \log n}$ so that Cole and Ramanchandran's \cite{ColeRamachandran} sorting algorithm can be run on them in $O(\log n)$ span. After running the Almost-Sort, the Full-Sort algorithm reincorporates all the elements that were set aside and due to a high probability guarantee on the number of these leftover elements, reincorporation dominates neither span or work.

Our approach for convex hulls differs in a few key ways:

1) We use convex hull algorithms at every level. We replace their $n^\epsilon$-way sort with angular elimination (described in Section \ref{sec:angular}). To match the workbound, we use angular elimination with $k=2$, giving us $O(n^{4/3} \log n)$ instead of $O(n^{3/2})$ work. We also replace the Cole and Ramachandran sorting algorithm with our adaptation, MultiwayMerge (described in Section \ref{sec:multiway}).

2) We bucket by angle, but when recursing over the said bucket, we find the envelope across the entire domain instead of just between bucket boundaries. For example, if we put points into the bucket for $[\pi/3, 3 \pi/4]$, then evaluating AlmostHull (our adaptation of Almost-Sort) on the next layer will still evaluate over the whole period $[0,2\pi)$. Only once all comparisons are made in the merge do we delete points that do not dominate in the bucket range. Additionally, when we place points into buckets, we are comparing with an envelope of a sample, so if the point's sinusoidal wave is completely dominated, we just discard it altogether.

3) We have to add in checks across buckets to make sure that points are constrained to those domains. In AlmostHull, this entails doing another run of the algorithm on conflicts, points that were placed in other buckets but after solving within the bucket they stretch into another buckets domain. These conflicts are placed in another array, and then the version in the conflict array is merged into the originals array. This merge can be done the same way that the pairwise merges are done in angular elimination, but since there are only two envelopes to compare for each bucket, it will be total $O(n)$ work. In  FullHull (our adaptation of Full-Sort), this entails checking across the bucket boundaries after using the MultiwayMerge, exactly as is done in that algorithm.

Otherwise, the algorithms are identical, and therefore the exact same probabilistic guarantees hold. In terms of collisions, the additional invocation of AlmostHull adds at most a constant factor. In fact, the collisions will in practice be likely significantly less as we will remove points from consideration if they are dominated by the envelope formed by the sample used for bucketing.


==> preliminaries.tex <==
\section{Preliminaries}\label{sec:preliminary}
In this paper, we use 2 different representations of the upper envelope of a set of sine waves. First, we are restricted to sine waves of the form $x \cos \theta + y \sin \theta$ as only these waves can be obtained from the Hough transform of a set of points. Therefore, all representations of the waves themselves are stored simply as tuples $(x,y)$.

\subsection{Vector-range form}
The first data structure is used in our algorithms is \textit{Vector-Range Form}, as it is the most intuitive. Every wave in the envelope has its vector representation, the range of angles over which it is in the envelope, its rank in the envelope, and the curve which succeeds it in rank order. These are usually stored in an array in rank order but can also be stored as a linked list.

\subsection{Primitives}
We use 5 primitive functions,  \textit{MaxVal}, \textit{ MaxSlope},  \textit{MaxToRight}, \textit{Intersections}, and \textit{CommonRange}. Each of them performs $O(1)$ work. We provide pseudocode for them in Appendix~\ref{sec:prim}, but it suffices to note that since their input sizes are constant, it is impossible for them to have greater time complexity than $O(1)$. 
\textit{MaxVal} and \textit{MinVal} return the wave of higher or lower value between the two input waves at a given angle.
\textit{MaxSlope} and \textit{MinSlope} do the same but for slope instead of value.
\textit{MaxToRight} and \textit{MaxToLeft} do the same as MaxVal but in case of a tie, they return the one which continues to be on top to the right and left of the given angle, respectively.
\textit{Intersections} determines the points of intersection between two input waves (where they cross each other).
\textit{CommonRange} determines the intersection of two intervals in $[0,2 \pi)$ (the range of angles common to both intervals).

\subsection{Positive curve form}

Another data structure we use is \textit{Positive Curve Form}. This structure maintains a list of angle-wave pairs which represent the upper envelope of a given set of sine waves and the x-axis (or $0 \cos \theta + 0 \sin \theta$). The result is an envelope for which only positive values are considered. 


\begin{figure*}
\centering
\begin{minipage}{\textwidth}
\centering
    \includegraphics[width=.6\textwidth]{images/hough transform.png}
%    \caption{Obtaining $R,\theta$ mapping for Hough Space}
    \caption{Length of the projection of a point $(x, y)$ on a straight line passing through the origin making $\theta$ angle with the horizontal axis is given by $l_{x,y, \theta} = x \cos{\theta} + y \sin{\theta}$ (the Hough curve). The perpendicular distance of the point from the line is given by $d_{x,y,\theta} = -x \sin{\theta} + y \cos{\theta}$ (another sinusoidal curve).}
    \label{fig:projection}
\end{minipage}
\\
\vspace{0.1in}
\begin{minipage}{0.4\textwidth}
    \centering
    \includegraphics[width=0.7\textwidth]{images/DAC representation singular- Copy (3).png}
    \caption{Positive Curve Form for split waves}
    \label{fig:singularsplit}
\end{minipage}
\hfill
\begin{minipage}{0.4\textwidth}
    \centering
    \includegraphics[width=0.7\textwidth]{images/DAC representation singular nonsplit.png}
    \caption{Positive Curve Form for non-split waves}
    \label{fig:singularnonsplit}
\end{minipage}\\
\vspace{0.1in}
\begin{minipage}{0.4\textwidth}
    \centering
    \includegraphics[width=.85\textwidth]{images/DAC representation envelope.png}
    \caption{Positive Curve Form for an upper envelope}
    \label{fig:envelope}
\end{minipage}
\hfill
\begin{minipage}{0.4\textwidth}
    \centering
    \includegraphics[width=.8\textwidth]{images/DAC representation empties.png}
    \caption{Positive Curve Form for an envelope with gaps}
    \label{fig:empties}
\end{minipage}\\
\vspace{0.1in}
\centering
\begin{minipage}{.9\textwidth}
    \centering
    \includegraphics[width=.7\textwidth]{images/sine point-line equivalence.png}
    \caption{Showing the relationship between Hough transform and point-line duality}
    \label{fig:equivalence}
\end{minipage}\\
\vspace{0.1in}
\centering
\begin{minipage}{0.65\textwidth}
    \centering
    \includegraphics[width=.8\textwidth]{images/DAC representation pivot- Copy.png}
    \vspace{-0.15in}
    \caption{Showing how the pivots work in Algorithms~\ref{alg:MultiwayMerge}}
    \label{fig:pivot}
\end{minipage}
\end{figure*}


An envelope with only a single wave is represented differently depending on where in the range $[0,2 \pi)$ it is above the x-axis. If a curve intersects the x-axis at $\theta_1, \theta_2$ where $\theta_1 < \theta_2$ and its value is negative for angles $\theta_1 < \theta < \theta_2$, then that is a "split waves". Split waves are represented as two separate waves, one for the $[0,\theta_1]$ component and the other for the $[\theta_2,2 \pi]$ component. See Figure 2 for an example. For non-split curves, we represent them as a single wave. See Figure 3 for an example


% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.3\textwidth]{images/DAC representation singular nonsplit.png}
%     \caption{Positive Curve Form for non-split waves}
%     \label{fig:singularnonsplit}
% \end{figure}

For each curve, we associate it in a pair with the first angle for which it is active. We also record the gaps where the x-axis dominates, with those being represented as an angle and a hyphen "-". Lastly, we record the end of an envelope with a "." and the angle $2 \pi$. These ends are not considered as waves by our algorithms. See Figures 4 and 5 for examples of upper envelopes.

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.3\textwidth]{images/DAC representation envelope.png}
%     \caption{Positive Curve Form for an upper envelope}
%     \label{fig:envelope}
% \end{figure}
% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.3\textwidth]{images/DAC representation empties.png}
%     \caption{Positive Curve Form for an envelope with gaps}
%     \label{fig:empties}
% \end{figure}

Unless stated otherwise, the algorithms in this paper use Vector-Range Form to represent the upper envelope. A curve can be converted from Vector-Range Form to Positive-Curve Form in constant time using the Intersections primitive with the wave $0 \cos \theta + 0 \sin \theta$ (the x-axis).

\subsection{Equivalence of transformations}

A common technique used in convex hull construction is finding the lower and upper envelopes of the dual representations of all the points under the standard point-line duality transformation. As opposed to our method of finding the upper envelope of sinusoidal curves, this method finds the upper envelope of lines. The advantage of using point-line duality is that there is no need to use trigonometric functions (which may take $\omega (1)$ work to compute with the required precision) to compute the relevant intersections along the envelope. However, using point-line duality requires two runs, one to find the upper envelope (corresponding to the lower hull) and one to find the lower envelope (corresponding to the upper hull).

For conceptual reasons, we use the sinusoidal model. However, our algorithms can be easily adapted to use point-line duality instead. This is because the relevant intersections along both envelopes are essentially the same. The two angles at which the sinuisoidal waves intersect correspond to a line coming from the origin which is perpendicular to the line formed by the two points. The intersection point in the dual plane for point-line duality translates back into the primal plane as the line formed by the two points. See Figure 5 for a demonstration of this.

Thus, instead of keeping track of the $\theta$ ranges for which a given wave is on top, we can instead keep track of the $-\cot \theta$ range for which a given wave would be on top to find the equivalent of the lower hull. This is because the negative cotangent of the angle is equal to the slope of the point-duality line, and the slope of that line is the x-value of the intersection point in the dual. This is essentially equivalent to taking the $r = a \cos \theta + b \sin \theta$ representation and dividing all by $-\sin \theta$ to get $\frac{r}{-\sin \theta} = a \cot \theta - b$, which is equivalent to the point-line duality transformation, $y = a x - b$.


==> prim.tex <==
\section{Primitives}\label{sec:prim}
We have several primitive functions which provide the basis for many of our algorithms presented. In the interest of implementation and completeness, we also provide pseudocode for them here.

\begin{algorithm}[ht]
\caption{MaxVal (For MinVal replace ">" with "<")}\label{alg:maxval}
\KwData{$w_1$ and $w_2$, two sine waves and $\theta$ an angle $[0,2 \pi]$}
\KwResult{The wave with the larger value at the angle}
\SetKwProg{Fn}{function}{:}{}
    \Fn{MaxVal($w_1,w_2, \theta$)}{
        $r_1 \gets w_1[x]\cos \theta + w_1[y] \sin \theta$\;
        $r_2 \gets w_2[x]\cos \theta + w_2[y] \sin \theta$\;
        \textbf{if} {$r_1 > r_2$} \textbf{then} {\Return $w_1$\;}
        \textbf{else} {\Return $w_2$\;}
    }
\end {algorithm}

\begin{algorithm}[ht]
\caption{MaxSlope (For MinSlope replace ">" with "<")}\label{alg:maxslop}
\SetKwProg{Fn}{function}{:}{}
\KwData{$w_1$ and $w_2$, two sine waves and $\theta$ an angle $[0,2 \pi]$}
\KwResult{The wave with the larger slope at the angle}
    \Fn{MaxSlope($w_1,w_2, \theta$)}{
        $r_1 \gets -w_1[x]\sin \theta + w_1[y] \cos \theta$\;
        $r_2 \gets -w_2[x]\sin \theta + w_2[y] \cos \theta$\;
        \textbf{if} {$r_1 > r_2$} \textbf{then} {\Return $w_1$\;}
        \textbf{else} {\Return $w_2$\;}
    }
\end{algorithm}

\begin{algorithm}[ht]
\SetKwProg{Fn}{function}{:}{}
\caption{MaxToRight (For MaxToLeft replace MaxSlope with MinSlope)}\label{alg:maxright}
\KwData{$w_1$ and $w_2$, two sine waves and $\theta$ an angle $[0,2 \pi]$}
\KwResult{The wave with the larger value at the angle and rightward}
    \Fn{MaxToRight($w_1,w_2, \theta$)}{
        $r_1 \gets w_1[x]\cos \theta + w_1[y] \sin \theta$\;
        $r_2 \gets w_2[x]\cos \theta + w_2[y] \sin \theta$\;
        \textbf{if} {$r_1 > r_2$} \textbf{then} {\Return $w_1$\;}
        \textbf{if} {$r_1 = r_2$} \textbf{then} {\Return MaxSlope($w_1,w_2, \theta$)\;}
        \textbf{else} {
        \Return $w_2$\;
        }
    }
\end{algorithm}

\begin{algorithm}[ht]
\caption{Intersections}\label{alg:intersections}
\SetKwProg{Fn}{function}{:}{}
\KwData{$w_1$ and $w_2$, two sine waves }
\KwResult{The angles $[0,2\pi)$ at which they intersect}
    \Fn{Intersections($w_1,w_2$)}{
        $\theta \gets \tan ^{-1} ( \frac{w_1[x] - w_2[x]}{w_2[y]-w_1[y]})$\;
        \textbf{if} {$\theta < 0$} \textbf{then} {
            $\theta \gets \theta + \pi$;
        }
        \Return $[\theta , \theta + \pi ]$\;
    }
\end{algorithm}

\begin{algorithm}[hb]
\SetKwProg{Fn}{function}{:}{}
\caption{CommonRange}\label{alg:commonRange}
\KwData{$I_1$ and $I_2$, two intervals $[0,2\pi)$}
\KwResult{The wave with the larger value at the angle}
\Fn{CommonRange($I_1,I_2$)}
    {
        \If{$I_1[0] < I_1[1]$}{ %%1
            \If{$I_2[0] < I_2[1]$}{ %%2
                $I \gets [\max (I_1[0], I_2[0]), \min (I_1[1],I_2[1])]$\;
                \textbf{if} {I[0] > I[1]} \textbf{then} { %3
                    \Return [0,0]\;
                }
                \textbf{else}{\Return I\;} %3
            }
            \Else{%2
                $I_2' \gets [0, I_2[1] - I_2[0] + 2\pi]$\;
                $I_1' \gets [I_1[0] - I_2[0] + 2\pi, I_1[1] - I_2[0] + 2\pi]$\;
                $I' \gets CommonRange(I_1',I_2')$\;
                \Return $ [I_2[0] + I'[0] \pmod{2 \pi}, I_2[0]+ I'[1]\pmod{2 \pi}]$\;
            }
            }
            
        \Else%1
        {
            \textbf{if} {$I_2[0] < I_2[1]$} \textbf{then} {%2
                \Return CommonRange($I_2, I_1$)\;    
            }
            \Else{%2
                $I_2' \gets [0, I_2[1] - I_2[0] + 2\pi]$\;
                $I_1' \gets [I_1[0] - I_2[0] + 2\pi, I_1[1] - I_2[0]  + 2\pi]$\;
                $I \gets CommonRange(I_2', I_1')$\;
                \Return $ [I_2[0] + I'[0] \pmod{2 \pi}, I_2[0]+ I'[1]\pmod{2 \pi}]$\;
            }
        }
    }
\end{algorithm}

==> pseudocodes.tex <==
\section{Algorithm Pseudocodes} \label{sec:pseudocodes}
We present pseudocode for the algorithms described above.

\begin{algorithm}
\small
\caption{Divide-and-Conquer with Multiway Merge}\label{alg:MultiwayMerge}
\KwData{$A$, a collection of sinusoidal envelopes, $L_1, L_2, ..., L_r$ where $n\leq 3r^6$}
\KwResult{The combined upper envelope of $A$}
\textbf{if} $n\leq 24$ \textbf{then} apply any serial upper envelope algorithm and return\;
\textbf{if} $n\leq 3r^3$ \textbf{then} $k \gets 1, A_1 \gets A$
\Else {
Form a sample $S$ of every $r^2$th curve (by associated angle) in each $L_i$, for a total of \shih{ $n/r^2$? what is $i$? what is $L_i?$}$n_i/r^2$ elements from each, where $n_i$ is the size of list $L_i$\;
Compute ranks of elements of $S$ using associated angle\;
Form a sample $P$ of every $2r$th member in $S$ by rank for a total of $\leq n/2r^3$ elements\;
Using $P$ as a set of pivots, partition $A$ into $k=|P|+1$ subsets ($A_1, ... A_k$). Include the curves which their right and left pivot angles pass through (See Figure 6)\; \shih{not quite sure. in this step, we have known the upper envelope? otherwise how can we use pivots like fig 6}
}
\textbf{parallel }\ForEach {subset $A_i$ of $A$ (from $1$ to $k$) }
{
    Separate $W_i$ into smaller subsets $A_{ij}$ such that each contains elements from at most $\sqrt{r}$ different lists\shih{$A_i \longrightarrow A_{ij}$: this is the recursion layer? define the list clearly. what is the range for $j$?}\;
    \textbf{parallel for each }$A_{ij}$ \textbf{do} MulitwayMerge($A_{ij}$) \; Run MulitwayMerge($A_i$) using the sorted $A_{ij}$ as lists\;
}
\textbf{parallel} \ForEach{pivot angle $p_i$ of $P$}{
    Determine the intersection angle between the last element of $A_i$ and the first element of $A_{i+1}$ and set the $A_{i+1}$ element's starting angle to it. 
}
\end{algorithm} 


\begin{algorithm}
\small
\caption{Dominating Range}\label{alg:DominatingRange}
\KwData{$W$, a set of $n$ sine waves of $x \cos(\theta) + y \sin(\theta)$, $wave$, another sine wave of the same form}
\KwResult{The range over which $wave$ dominates $W$ and the wave that dominates it to the right}

\If {W.size = 1} {
		$I \gets Intersections(wave, W[0])$\;
		$S.next \gets W[0]$\;
		\textbf{if} {wave $\neq$ MaxToRight(I[0])} \textbf{then} {
		    $I \gets[ I[1], I[0]]$\;
			
			}
    $S.range \gets I$\;
    \Return S\; 
    }
$W_1 \gets [W[0] ... W[n/2-1]]$\;
$W_2 \gets [W[n/2]...W[n-1]]$\;
\textbf{spawn}\;
\textbf{if} {new thread} \textbf{then} {
$S_1 \gets DominatingRange(W_1,n/2,wave)$\;
}
\textbf{else} {
	$S_2 \gets DominatingRange(W_2,n/2,wave)$\;
	}
$S.range \gets CommonRange(S_1.range, S_2.range)$\;
$S.next \gets MaxVal(S_1.next,S_2.next, S.range[1])$\;
\Return S\;


\end{algorithm}


\begin{algorithm}
\small
\caption{Base Case for Angular Elimination}\label{alg:baseAngularElimination}
\KwData{$W$, a set of $n$ sine waves of $x \cos(\theta) + y \sin(\theta)$}
\KwResult{The upper envelope of $W$}
\SetKwProg{Fn}{function}{:}{}
    \textbf{parallel} \ForEach{wave in W} {
		$IntersectInfo = DominatingRange(W,n,wave)$\;
		$wave.range = IntersectInfo.range$\;
		$wave.next = IntersectInfo.range$\;
		\textbf{if} {wave.range is empty} \textbf{then} {$wave.rank \gets n$}\;
		\textbf{else} {
		    $wave.rank \gets 0$;
		}
		}
	ListRanking(W)\;
	$E = $ array of size n\;
	\textbf{parallel} \ForEach {wave in W}{
		\textbf{if} {wave.rank < n} \textbf{then} {
			E[wave.rank] = wave\;
		}
	    }
	\Return E\;
\end{algorithm}


\begin{algorithm}
\small
\caption{Angular Elimination}\label{alg:angularElimination}
\KwData{$W$, a set of $n$ sine waves of the form $x \cos(\theta) + y \sin(\theta)$, a parameter k}
\KwResult{The upper envelope of $W$}
\textbf{if} {$k \leq 1$} \textbf{then} {
    \Return BaseCase(S,n)\;
}
\textbf{parallel} \ForEach {subset S of size $n^{(k-1)/k}$} {
	 $S \gets Angular Elimination(S,n^{(k-1)/k},k-1)$\;
	}
\textbf{parallel} \ForEach {wave in W} {
	$P \gets$ array of size $n^{\frac{1}{k}}$\;
	\textbf{parallel} \ForEach {envelope S in P} {
		$L \gets $ the curve in S containing wave.range[0]\;
		$R \gets $ the curve in S containing wave.range[1]\;
		$W_i \gets $ the curves of S between L and R\;
		$P[i] \gets DominatingRange(W_i,n^{\frac{k-1}{k}},wave)$\;}
$wave.range \gets $ \textit{CommonRange} among all P[i].range\;
$wave.next \gets $ \textit{MaxToRight} among all P[i].next\;
\textbf{if} {wave.range is empty} \textbf{then} {$wave.rank \gets n$}\;
		\textbf{else} {
		    $wave.rank \gets 0$;
		}
}
	$ListRanking(W)$\;
	$E \gets $array of size n\;
	\textbf{parallel} \ForEach{wave in W}{
		\textbf{if} {wave.rank < n} \textbf{then} {
			$E[wave.rank] \gets wave$\;
		}
	}
	\Return E;
\end{algorithm}


\begin{algorithm}
\small
\caption{AlmostHull}\label{alg:almosthull}
\KwData{$B$, a set of sine waves of the form $x \cos \theta + y \sin \theta$,\\ $n_c$ : size of array to sort (only $B[l_0, ..., l_0 + nc - 1]$ is occupied)\\
$n$ : size of the array at the highest level of recursion\\
$l_0$ : location where the array to sort begins\\
$d$ : depth of current call in recursion tree\\
$m$ : multiple of extra memory to use\\
$B[l_0, ..., l0 + n_cm - 1]$ : contains array to be sorted\\
$C[l_0, ..., l0 + n_cm - 1]$ : ancillary space\\
$C_2[l_0, ..., l0 + n_cm - 1]$ : secondary ancillary space\\
$D[l_0, ..., l0 + n_cm - 1]$ : where prefix sums will be stored (for indexing)}
\KwResult{The upper envelope of $W$}
\textbf{if $d \geq \log \log \log n$ then return} $MultiwayMerge(B[l_0, l_0 + n_c -1]$\;
$s \gets \log ^3 n_c$\;
$P \gets$ sample with repetition of size $(\sqrt{n_c}+1)s$ from $B[l_0, l_0 + n_c -1]$\;
$P \gets AngularElimination(P,3)$\;
$P[0] \gets 0, P[(\sqrt{n_c}+1)s] \gets 2\pi$\;
Space out the elements of P as evenly as possible. Fill the gaps with duplicates of the points but with split ranges\;
\{ Bucketing \} \\
\textbf{parallel }\ForEach{$a \in B[l_0, l_0 + n_c -1]$}{
Find some $i$ where $a$ begins dominating the pivot envelope between $P[i\cdot s]$ and $P[(i+1) \cdot s$\, if none exists do nothing;
Choose a random number $j \in [0, ... m \sqrt{n_c}-1$\;
Attempt $C[im \sqrt{n_c} + j] \gets a$, doing nothing if collision
}
\textbf{parallel for } $i \gets l_0$ to $l_0 + n_c -1$ \textbf{do} $B[i] \gets$ null \;
\{Compacting\}\\
\textbf{parallel} \ForEach{$i \in [0, n_c - 1$}{
    $\text{low} \gets l_0 + im \sqrt{n_c}$\;
    $\text{hi} \gets l_0 + (i+1) m \sqrt{n_c}-1$\;
    $D[\text{low},\text{hi}] \gets \text{Indicator-Prefix-Sum}(C[\text{low},\text{hi})$\;
    \textbf{parallel} \ForEach{$j \in [\text{low},...\text{hi}]$}{
        $D[j] = D[j] + im \sqrt{n_c}$\;
    }
}
\textbf{parallel} \ForEach{$i \in [l_0, l_0 + n_c m - 1$}{
    \If{$C[i]$ is not null}{
        $B[D[i]] \gets C[i]$\;
        $C[i] \gets$ null\;
    }
}
\{Solving Buckets and Comparing \}\\
\textbf{parallel} \ForEach{$i \in [0, ... \sqrt{n_c}-1]$}{
    AlmostHull($\sqrt{n_c},n,l_0 +im \sqrt{n_c}, d+1, m, B, C, D$)\;
}
\textbf{parallel} \ForEach{$i \in [0, ... \sqrt{n_c}-1]$}{
    \textbf{parallel} \ForEach{$j \in [0, ... \sqrt{n_c}-1]$}{
        \textbf{if} $i = j$ \textbf{then} do nothing\;
        Determine if the $ith$ bucket envelope dominates the $jth$ bucket within its bucket. If so, randomly assign it to a corresponding slot in $C_2$ (just as before, do nothing if already occupied).
    }
}
\textbf{parallel} \ForEach{$i \in [0, ... \sqrt{n_c}-1]$}{
    Use AlmostHull on the bucket conflicts in $C_2$, then merge the conflict bucket with the original bucket.
}
$C \gets B$; $D \gets \text{Indicator-Prefix-Sum}(C)$\;

\textbf{parallel for } $i \in [0,...n_cm-1]$ \textbf{do if} $C[i]$ is not null \textbf{then} $B[D[i] \gets C[i]$
\end{algorithm} 



\begin{algorithm}
\footnotesize
\caption{Full-Hull}\label{alg:fullhull}
\KwData{$A$, a set of sine waves of the form $x \cos \theta + y \sin \theta$}
\KwResult{The upper envelope of $W$}
$m \gets \log n \log \log \log n/ \log \log n$; Allocate arrays $B, C, C_2, D $ of size $nm$; $B[0, ..., n - 1] \gets A$\;
$Almost-Hull(n, n, 0, 0, m, B, C,C_2, D)$\;
$\text{num\_sorted} \gets $ smallest $i$ s.t. $B[i] = $ null\;
Set all elements of C and D to null\;
Allocate arrays E, F of size n \;
\textbf{parallel} \ForEach{$a \in A[0, ... , n-1]$}{
    Find smallest $i$ s.t. $B[i] \leq a < B[i+1]$ (comparing start angle)\;
    \If {$a \neq B[i]$} {
        Choose a random number $j \in [0, ... , m-1]$\;
        Attempt $C[i\cdot m +j] \gets a$; do nothing if collision\;
    }
}
$D \gets $ Indicator-Prefix-Sum($C$)\;
\textbf{parallel} \ForEach{$i \in [0,...n]$}{
    \textbf{if} $D[i\cdot \text{block\_size}] \neq D[(i+1)\cdot \text{block\_size} -1$ \textbf{then E[i] = 1}\l
}
$F \gets Prefix-Sum(E)$\;
Set all elements of C and D to null\;
$\text{block\_size} \gets log^3 n log^2
log log n/ log^3\log n$\;
\textbf{parallel} \ForEach{$a \in A[0, ... , n-1]$}{
    Find smallest $i$ s.t. $B[i] \leq a < B[i+1]$, (comparing start angle)\; 
    \If {$a \neq B[i]$\textbf{ and }$E[i] = 1$} {
        Choose a random number $j \in [0, ... , \text{block\_size}-1]$\;
        Attempt $C[(F[i]-1)\cdot \text{block\_size} +j] \gets a$; do nothing if collision\;
    }
}
$D \gets $ Indicator-Prefix-Sum($C$)\;
\textbf{parallel} \ForEach{$i \in [0, ... \text{num\_sorted}-1$}{
    \textbf{if} $E[i]=0$ \textbf{then $E[i] = 1$}\;
    \textbf{else} $E[i] = D[F[i]\cdot \text{block\_size}-1] - D[F[i]$
    }
Set all elements of C and D to null\;
\textbf{parallel} \ForEach{$i \in [0,...n-1]$}{
\textbf{parallel} \ForEach{$j \in [0, \log n - 1$}{
    Choose a random number $k = H(j, (F[i]-E[i])m, F[i]m -1)$\;
    Attempt $C[k] \gets a$; do nothing if collision\;
}
chunk\_size $\gets n \log \log \log n / \log \log n$\;
\ForEach{$i \in [0, ... n/\text{chunk\_size}-1$}{
    \textbf{parallel} \ForEach{$a \in A[i\cdot \text{chunk\_size},...,(i+1)\cdot  \text{chunk\_size} -1$}{
        Find smallest $i$ s.t $B[i] \leq a < B[i+1]$ (comparing start angle)\;
        Keep-Single(C,a,n,H,(F[i]-E[i])m, F[i]m -1)
    }
}
}
\textbf{parallel} \ForEach{$i\in {0,...\text{num\_sorted}-1}$}
{
    $D[(F[i]-E[i])m,...F[i]m-1] \gets$ Indicator-Prefix-Sum(C[(F[i]-E[i])m,..., F[i]m -1])\;
    \textbf{parallel} \ForEach{$j \in [(F[i]-E[i])m, F[i]m -1]$}{
        $D[j] \gets D[j] + (F[i]-E[i])m$\;
    }
}
\textbf{parallel} \ForEach{$i \in [0, ... nm-1]$}{
    \textbf{if} $C[i] \neq $ null \textbf{then} \{$A[D[i]] \gets C[i]; C[i] \gets null$\}
    }
\textbf{parallel} \ForEach{$i \in [0,...\text{num\_sorted}-1]$}{
    lo $\gets (F[i]-E[i])m$; hi $\gets$ lo $+E[i]$\;
    $A[$lo,.., hi$] \gets $ Multiway-Merge($A[$lo,.., hi$]$)\;
}
\textbf{parallel} \ForEach{$i \in [0,...\text{num\_sorted}-1]$}{
    lo $\gets (F[i]-E[i])m$; hi $\gets$ lo $+E[i]$\;
    Check across boundaries of lo and hi to adjust start positions.
}
$D \gets$ Indicator-Prefix-Sum(A)\;
\textbf{parallel for} $i \in [0,...nm-1]$ \textbf{do if } $A[i] \neq$ null \textbf{then} {$C[D[i]]\gets A[i]; A[i] \gets $ null;}\;
$A \gets C$\;
\end{algorithm} 

==> relatedWorks.tex <==
\section{Related Work}\label{sec:related}

% Related Works
Considering non-output-sensitive serial algorithms, the best running time that can be reached is $O(n\log n)$. Graham Scan~\cite{Graham1972AnEA} was the first algorithm that achieves this optimal running time. There are several other approaches proposed afterward that have the same running time as well \cite{ANDREW1979216, Preparata1977, barber1996quickhull, kallay1984complexity}. For the output-sensitive serial algorithms, the Gift Wrapping method achieves a running time of $O(nh)$~\cite{JARVIS197318}, which was later improved to $O(n \log h)$~\cite{kirkpatrick1986ultimate, ChanAlgorithm}. 

Efficient convex hull algorithms have been designed in various parallel models. With presorted input, the optimal bound of span and work in PRAM models are ($O(\log n)$, $O(n)$) (the first element of this tuple represents the asymptotic span bound and the second one represents the asymptotic work bound) in the EREW (exclusive reads and writes) model \cite{yu1995efficient} and ($O(\log \log n)$, $O(n)$) in the CRCW (concurrent reads and writes) model \cite{berkman1996fast}. For the unsorted input, the optimal span is $O(\log n)$ and work is $O(n \log h)$ in the EREW model~\cite{miller1988efficient} and randomized CRCW with n-exponential probability~\cite{ghouse1997fast}. 

A randomized incremental convex hull algorithm is the first to be analyzed in binary-forking model~\cite{blelloch2020randomized}. It performs $O(n\log n)$ expected work. Its span is $O(\log n \log^{*} n)$ in PRAM model and $O(\log ^2n)$ in the binary-forking model with high probability in $n$.
%
There have been a recent surge of interest in designing parallel algorithms for solving various problems on variants of the binary-forking model~\cite{ColeRamachandran,ramachandran2021data,BlellochFiGuSu2019,CooleyTu65,goodrich2021atomic,ahmad}
